Integral Hilbert spaces and the dynamics of loop quantum cosmos

Polymer quantization program applied in Loop Quantum Gravity/Cosmology leads to nonseparable Hilbert spaces. Commonly, one sidesteps this problem by singling out and working with a separable superselection sector. This is however often no longer accessible in more involved models beyond isotropic ones. In an alternative approach one builds a separable Hilbert space as an integral over all available sectors. Here we test the dynamics following from the latter on the example of a flat isotropic Universe admitting negative cosmological constant and a massless scalar field. There, numerical evolution of (initially) semiclassical states shows that there is no relevant difference in their long term semiclassicality properties in comparison to those in a single sector approach. Further, the older (problem-specific) numerical methods are compared against an application of more common and more efficient standard tools (eigen library).

==> makefile <==

all:
	pdflatex main.tex && bibtex main && pdflatex main.tex && pdflatex main.tex

clean:
	rm -f main.aux main.bbl main.blg main.log main.spl main.out mainNotes.bib

# Co sekundę sprawdza datę tego katalogu i jeśli jakiś plik się zmienił to kompiluje.
watchCompile:
	while true;do bash ./watch.sh || /usr/bin/time -f "\n\tCompile time: %E" make warn; sleep 1; done

warn:
	${MAKE} all 2>&1 | grep -v fancyhdr | grep -v hyperref | grep --color=always -iE "error:|warning|^l\..*" -A 3 -B 1 || true
	touch /tmp/67bf20d3c_make



